Prompt Generation Networks for Input-Space Adaptation of Frozen Vision Transformers

With the introduction of the transformer architecture in computer vision, increasing model scale has been demonstrated as a clear path to achieving performance and robustness gains. However, with model parameter counts reaching the billions, classical finetuning approaches are becoming increasingly limiting and even unfeasible when models become hosted as inference APIs, as in NLP. Visual input-prompt learning, an adaptation technique in which additional inputs in visual (RGB) space are learned, has emerged as a potential solution for adapting frozen and cloud-hosted models, requiring neither access to the forward pass, nor post-processing. Yet so far, these constraints have deteriorated adaptation performances significantly. To this end, we propose the Prompt Generation Network (PGN) that generates a different prompt for every data point, which is then used to adapt a frozen pretrained vision model to a target task. We show that the PGN effectively adapts pretrained models to various new datasets: It surpasses previous methods by a large margin on 12/12 datasets and even outperforms full-finetuning on 5/12, while requiring 100x fewer parameters. Lastly, we introduce the "prompt inversion" trick, with which PGNs can be efficiently trained in a latent space but deployed in RGB input space for inference.

==> figures/attention_histogram.tex <==
% \begin{figure}[h]
    \begin{center}
    \includegraphics[width=\textwidth]{images/att_hist_flat.png}
    \end{center}
    \vspace{0.5em}
    \caption{\textbf{Attention value histograms.} We show the individual attention values from the \texttt{CLS} token to the supplied prompts of PGN and IIP.
    We find that while PGN has an overall lower average attention, the input-dependency successfully yields a wider distribution in adapting the original model.
    \label{fig:attention_histogram}}
% \end{figure}

==> tables/abl_method.tex <==
% \begin{table}[]
    \begin{center}
    \vspace{-0.5em}
    \label{abl_method}
    \setlength\tabcolsep{0.22em}
    \begin{small}
    \begin{tabular}{lccccc}
        \toprule
                 & CIFAR100 & SUN397 & \#{}params & FLOPs & throughput\\
        \midrule
        Direct     & 79.0  & 70.8  & \textit{3.2M} & 5.6 $\times 10^8$ & 401 $s^{-1}$\\
        \textbf{TL}& 79.3  & 70.6  & \textit{0.3M} & 5.6 $\times 10^8$ & 398 $s^{-1}$\\
        \bottomrule
    \end{tabular}
    \vspace{-2mm}
            \captionof{table}{\textbf{Similar performances but less parameters.} The Token Library (TL) achieves comparable results compared to direct generation of prompts, but only requires a fraction of the added parameters. 
            Reported results are obtained for $8$ prompts and a token library of $64$. 
    %, which gives PGNs of 312K (TL) and 3.15M (direct) parameters.
    }
    \end{small}
    \end{center}
% \end{table}






% % \begin{table}[]
%     \begin{center}
%         \captionof{table}{\textbf{Similar performances.} The Token Library (TL) achieves comparable results compared to direct generation of prompts, but only requires a fraction of the added parameters. Reported results are obtained for $8$ prompts and a token library of $64$. 
%     %, which gives PGNs of 312K (TL) and 3.15M (direct) parameters.
%     }
%     \vspace{-1em}
%     \label{abl_method}
%     \setlength\tabcolsep{0.55em}
%     \begin{small}
%     \begin{tabular}{lcc}
%         \\\toprule
%                  & Direct & \textbf{TL} \\
%         \midrule
%         CIFAR100 & 79.0 & 79.3 \\
%         SUN397 & 70.8 & 70.6 \\
%         \textit{\#{}parameters} & \textit{3.2M} & \textit{0.3M} \\ 
%         \bottomrule
%     \end{tabular}

%     \end{small}
%     \end{center}
%     \vskip -0.1in
% % \end{table}

==> tables/att_statistics.tex <==
\begin{table}[h]
    \begin{center}
    \caption{Comparison of the attention submatrices of CLIP and PGN-CLIP, specified by query and key type. Each value is a sum over key elements and averaged over all heads and layers of CLIPs image encoder and 1000 SUN397 test points.}
    \label{att_statistics}
    \setlength\tabcolsep{0.3em}
    \begin{small}
    \begin{tabular}{lccc}
        \\ \toprule
        Query & Key & CLIP & PGN \\
        \midrule
        CLS & prompt & - & 0.274 \\
        patch & prompt & - & 0.140  \\
        \midrule
        patch & CLS & 0.292 & 0.228 \\
        CLS & patch & 0.396 & 0.263 \\
        \bottomrule
    \end{tabular}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table}

==> tables/combined_dataset.tex <==
\begin{table}[h]
    \begin{center}
    \captionof{table}{Multi dataset}
    \label{abl_architecture}
    \setlength\tabcolsep{0.3em}
    \begin{small}
    \begin{tabular}{lccc}
        \toprule
        Dataset & Individual & Comb1 & Comb2 \\
        \midrule
        EuroSAT & 98.0 & 97.0 & 95.8 \\
        UCF101 & 77.7 & 73.0 & 73.6\\
        Resisc45 & 92.3 & 90.1 & 87.7 \\
        Pets & 91.5 & 89.0 & 88.4 \\
        CIFAR100 & 79.3 & - & 73.3\\
        \bottomrule
    \end{tabular}
    \end{small}
    \end{center}
    \vskip -0.1in
\end{table}
